Where Should Robotaxis Operate? Strategic Network Design for Autonomous Mobility-on-Demand

The emergence of Autonomous Mobility-on-Demand (AMoD) services creates new opportunities to improve the efficiency and reliability of on-demand mobility systems. Unlike human-driven Mobility-on-Demand (MoD), AMoD enables fully centralized fleet control, but it also requires appropriate infrastructure, so that vehicles can operate safely only on a suitably instrumented subnetwork of the roads. Most existing AMoD research focuses on fleet control (matching, rebalancing, ridepooling) on a fixed road network and does not address the joint design of the service network and fleet capacity. In this paper, we formalize this strategic design problem as the Autonomous Mobility-on-Demand Network Design Problem (AMoD-NDP), in which an operator selects an operation subnetwork and routes all passengers, subject to infrastructure and fleet constraints and route-level quality-of-service requirements. We propose a path-based mixed-integer formulation of the AMoD-NDP and develop a column-generation-based algorithm that scales to city-sized networks. The master problem optimizes over a restricted set of paths, while the pricing problem reduces to an elementary shortest path with resource constraints, solved exactly by a tailored label-correcting algorithm. The method provides an explicit certificate of the optimality gap and extends naturally to a robust counterpart under box uncertainty in travel times and demand. Using real-world data from Manhattan, New York City, we show that the framework produces stable and interpretable operation subnetworks, quantifies trade-offs between infrastructure investment and fleet time, and accommodates additional path-level constraints, such as limits on left turns as a proxy for operational risk. These results illustrate how the proposed approach can support strategic planning and policy analysis for future AMoD deployments.

==> chapters/definition.tex <==
\section{OLD:Problem Definition} \label{sec:pd}
In this section, we formally define the \gls{acr:andp}. We first introduce core concepts for the system and problem representation, which enable the formulation of the network design problem later. 
The \gls{acr:andp} involves designing an operation network within a base road transportation network. The operation betwork is a sub-network of the base road network that defines the region where the \gls{acr:amod} service operates. We begin by defining essential concepts related to the system setup: the base road network, demand, and the demand-satisfactory path.

\begin{definition}[Base Road Network] The base road transportation network is represented by a directed graph $\mathcal{G} = (\mathcal{V},\mathcal{E})$, where $\mathcal{V}$ is the set of nodes and $\mathcal{E} \subseteq \mathcal{V} \times \mathcal{V}$ the set of directed edges. Define two maps $s: \mathcal{E} \rightarrow \mathcal{V}$ and $t: \mathcal{E} \rightarrow \mathcal{V}$ that assign an edge $e \in \mathcal{E}$ to its source and sink nodes. Only one edge $e \in \mathcal{E}$ exists between the source and sink nodes $s(e)$ and $t(e)$. 

Each edge on $\mathcal{G}$ is associated with a vector of time-independent attributes. Let $\mathcal{I}:= \{1,\dots, n\}$ be the index set of edge attributes. The vector of attributes for edge $e$ is
\[A(e) = (A_1(e), ..., A_n(e)) \in \mathcal{A}_1 \times \dots \times \mathcal{A}_n,\]
where each $\mathcal{A}_i$ denotes the codomain of attribute $i$. The map $A_i: \mathcal{E} \rightarrow \mathcal{A}_i$ returns attribute $i$ of edge $e$. In particular, the attribute maps giving travel time and distance are denoted by $T: \mathcal{E} \rightarrow \mathbb{R}_{>0}$ and $L: \mathcal{E} \rightarrow \mathbb{R}_{>0}$.
\end{definition}

The demand in the system is represented by a set of \gls{acr:od} pairs defined as follows.
\begin{definition}[Demand] For any ordered pair of distinct nodes $(i,j) \in \mathcal{V} \times \mathcal{V}$ with $i \neq j$, let $d_{ij} := (i,j,\alpha_{ij})$ denote the travel demand from origin $i$ to destination $j$, where $\alpha_{ij} \in \mathbb{R}_{>0}$ is the number of travelers wishing to move from $i$ to $j$. The total demand is defined as the set of all \gls{acr:od} demands with a positive number of travelers $\mathcal{D}:=\{d_{ij}|i,j \in \mathcal{V},i \neq j, \alpha_{ij} > 0\}$.
\end{definition}

The demands are satisfied by following paths between the corresponding origin and destination on the operation network. 
\begin{definition}[Path] Assume $i, j$ are two distinct nodes. A path from $i$ to $j$ can be represented in either of the following equivalent forms:
\begin{enumerate}
    \item An ordered node sequence $p:=(v_1, \dots, v_l)$ such that $v_1 = i$, $v_l = j$, and $(v_k,v_{k+1}) \in \mathcal{E}$ for all $k = 1, \dots, l-1$.
    \item An ordered edge sequence $p:=(e_1, \dots, e_{l-1})$ such that $t(e_k)=s(e_{k+1})$ for all $k = 1, \dots, l-2$ if $l > 2$. When $l = 2$, the path collapses into a single-edge path.
\end{enumerate}
\end{definition}

\begin{remark}
    The node-sequence and edge-sequence representations are one-to-one correspondence: each node path uniquely determines an edge path, and vice versa.
\end{remark}

\begin{definition}[Demand-Satisfactory Path]
A path with node-sequence representation $p := (v_1, \dots, v_l)$ is a demand satisfactory path if $v_1 = i, v_l = j$ for some $d_{ij} \in \mathcal{D}$.
    
\end{definition}

Based on the above definitions, a general \gls{acr:andp} is defined as follows.

\begin{definition}[\gls{acr:andp}] \label{def:ndp} On a base road network $\mathcal{G}$ with demand profile $\mathcal{D}$, the \gls{acr:amod} network design problem is presented as an optimization problem that optimizes certain system functionality
\[F(\mathbf{x},\mathbf{y})\]
by designing $\mathbf{x}$ and $\mathbf{y}$, which are decisions on:
\begin{enumerate}
    \item $\mathbf{x}:=(x_1,\dots, x_{|\mathcal{E}|})$ is a vector where each element $x_i \in \{0,1\}$ represents the decision of either instrumenting edge $i$ to enable safe autonomous driving.
    \item $\mathbf{y}:=(y_1, \dots, y_{|\mathcal{E}|})$ is a vector where each element $y_i \in \mathbb{R}$ represents the optimal passenger flow on edge $i$ that optimizes $F(x,y)$ based on the network structure decided by $\mathbf{x}$.
\end{enumerate}
The edge instrumentation is subject to a limited budget $B$, which is represented by
\[\mathbf{b}^T \mathbf{x} \leq B\]
where each element $b_i$ in the vector $\mathbf{b}$ denotes the cost of instrumenting edge $b_i$. The flow distribution is subject to some resource constraint:
\[\mathbf{r}^T \mathbf{y} \leq R\]
where each element $r_i$ in the vector $\mathbf{r}$ denotes the resource consumed to transport one unit of flow on the edge. The flows on edges are also subject to a limited road capacity constraint
\[\mathbf{y} \leq \mathbf{c}\]
where each element $c_i$ in the vector $\mathbf{c}$ denotes the edge capacity.
\end{definition}

In this work, we focus on one type of \gls{acr:andp} that satisfies the following assumption.

\begin{assumption} \label{assump:link}
    The functionality is calculated based on the flow vector $\mathbf{y}$, and $F(\mathbf{y})$ is link-separable, i.e.,
    \[F(\mathbf{y}) = \sum_{i \in \{1,\dots,|\mathcal{E}|\}}F_i(y_i)\]
    where $F_i:\mathbb{R}_{+}\to\mathbb{R}$ quantifies the contribution of edge $i$ as a function of its flow $y_i$.
\end{assumption}

Assumption~\ref{assump:link} is s standard additive structure used when system-level performance can be expressed as a sum of local costs or rewards accrued along a path. Concretely, if each unit of flow traversing edge $i$ incurs a cost (or yields a reward) that depends only on the amount of flow on that edge, then the total system functionality is obtained by aggregating these per-edge contributions, which leads directly to link separability.

This structure captures several commonly used objective terms regarding transportation system performance. For example, total travel distance can be written as $\sum_i y_i\, L(i)$. Similarly, objectives that approximate operational cost by distance- or time-proportional charges also decompose into per-edge terms. A profit-related objective inherits the same additivity when revenue and marginal operating cost are computed as a sum of edge-level components, which is a common practice in on-demand mobility services. In all of these cases, interactions across edges enter only through the feasibility conditions (flow conservation, capacity, and resource constraints), while the objective itself remains a sum of single-edge functions.

At the same time, Assumption~\ref{assump:link} excludes important classes of objectives and constraints that are inherently path-dependent or nonlocal, such as penalties on end-to-end travel time, guarantees on path reliability, risk exposure along a trajectory, or any metric that depends on the specific sequence of edges rather than on the marginal flows alone. Later, we discuss how the proposed modeling and solution approach can be extended to accommodate such non-separable, path-dependent specifications.

\begin{assumption} \label{assump:linear}
    $F_i$ is an affine function, i.e.
    \[F_i(y_i) = \beta_i^0 + \beta_i \cdot y_i\]
\end{assumption}

Assumption~\ref{assump:linear} models functionality as an additive baseline term plus a marginal contribution that scales proportionally with the amount of flow on edge $i$. This approximation is standard in the system design phase when (i) one wishes to approximate the measure of functionality by aggregated usage and (ii) the marginal benefit (or marginal cost, if $\beta_i<0$) per unit flow is taken to be an expected constant value over the operating range of interest.

\begin{lemma}[Irrelevance of the intercept term]
    The intercept in $F_i$ does not influence the optimal solution of the \gls{acr:andp}.
\end{lemma}
\begin{proof}
    Assume that there are two \gls{acr:andp}s $I_1$ and $I_2$ with the objective of maximizing functionality. These two problems only differ in the functions for computing functionality, where for $I_1$, $F_i^1(y_i)= \beta_i \cdot y_i$, and for $I_2$, $F_i^2(y_i)=\beta_i^0 + \beta_i \cdot y_i$. Denote the optimal solution for $I_1$ as $(\mathbf{x}^*, \mathbf{y}^*)$, for any legitimate solution $(\mathbf{x},\mathbf{y}) \neq (\mathbf{x}^*, \mathbf{y}^*)$, the following inequality holds by definition:
    \[\sum_{i \in \{1,\dots,|\mathcal{E}|\}}F^1_i(y_i) \leq \sum_{i \in \{1,\dots,|\mathcal{E}|\}}F^1_i(y_i^*)\]

    Then we can also get:
    \begin{align*}
        \sum_{i \in \{1,\dots,|\mathcal{E}|\}}F^2_i(y_i) &= \sum_{i \in \{1,\dots,|\mathcal{E}|\}}F^1_i(y_i) + |\mathcal{E}|\cdot\beta_i^0 \\
        &\leq \sum_{i \in \{1,\dots,|\mathcal{E}|\}}F^1_i(y_i^*) + |\mathcal{E}|\cdot\beta_i^0 \\
        &= \sum_{i \in \{1,\dots,|\mathcal{E}|\}}F^2_i(y_i^*)
    \end{align*}
    $(\mathbf{x}^*, \mathbf{y}^*)$ is also the optimal solution for $I_2$. Therefore, the intercept $\beta_0$ does not influence the optimal solution of the problem.
\end{proof}

For simplified notation, in the rest of the manuscript, we assume that $F_i$ follows the format of $F_i(y_i) = \beta_i \cdot y_i$.
